New Physics at the TeV Scale

The Standard Model of particle physics is assumed to be a low-energy effective theory with new physics theoretically motivated to be around TeV scale. The dissertation presents theories with new physics beyond the Standard Model at the TeV scale testable in the current High Energy Colliders. The study on leptoquarks gauge bosons in reference to TopSU(5) model in chapter 2 showed that their discovery mass range extends upto 1.5 TeV at 14 TeV LHC with luminosity of 100 $fb^{-1}$. On the other hand, in chapter 3 we studied the collider phenomenology of TeV scale mirror fermions in Left-Right Mirror model finding that the reaches for the mirror quarks goes upto $750$ GeV at the $14$ TeV LHC with $~300 ~fb^{-1}$ luminosity. In chapter 4 we have enlarged the bosonic symmetry to fermi-bose symmetry e.g. supersymmetry and have shown that SUSY with non-universalities in gaugino or scalar masses within high scale SUGRA set up can still be accessible at LHC with 14 TeV. In chapter 5, we performed a study in respect to the $e^+e^-$ collider and find that precise measurements of the higgs boson mass splittings upto $\sim 100$ MeV may be possible with high luminosity in the International Linear Collider (ILC). In chapter 6 we have shown that the experimental data on neutrino masses and mixings are consistent with the proposed 4/5 parameter Dirac neutrino models yielding a solution for the neutrino masses with inverted mass hierarchy and large CP violating phase $\delta$ and thus can be tested experimentally. Chapter 7 incorporates a warm dark matter candidate in context of two Higgs doublet model. The model has several testable consequences at LHC. This dissertation presents an endeavor to study beyond standard model (BSM) physics at the TeV scale with testable signals in the Colliders.

==> SMextra.tex <==
%
% chapter 1 : Introduction
%
\chapter{\label{CH_INTRO} Introduction }

    In the standard model of elementary particle physics, quarks and leptons
    interact via the exchange of photons and intermediate vector bosons,
    as described by the Glashow-Weinberg-Salam standard model of weak
    interactions \cite{WEINBERG,SALAM,GLASHOW}. 
    In addition, quarks are subject to the strong interaction, 
    described by quantum chromodynamics (QCD) \cite{QCD}.

    The area of interest for this analysis is the
    transformation of quarks and gluons into observable hadrons
    (parton fragmentation) in high energy reactions.
    This transformation is governed by QCD which is predictive in
    high energy processes where perturbation theory can be used.
    However, the final stage of the transformation (hadronisation)
    occurs at low energy where perturbation theory is no longer applicable,
    therefore phenomenological models are constructed to describe the
    hadronisation.

    A clean environment for the study of fragmentation has been provided
    by the Large Electron Positron Collider (LEP) in which the process 
    $\ee \rightarrow Z \rightarrow q \bar{q}$
    can be selected with little contamination from background processes.
    Measurements of the hadronic final state are made in order to test the
    fragmentation models: parameters in the models are tuned to
    reproduce observed distributions such as event shape variables,
    jet production rates, and particle production rates.

    The area of analysis presented in this thesis is inclusive particle
    production. Many particle species have been measured in previous
    $\ee$ annihilation experiments and a number of \MC programs based on 
    QCD have been tuned so that the measured rates were reproduced.
    A comprehensive compilation of experimental 
    data on inclusive particle production in $\ee$ interactions can be found 
    in \cite{LAFFERTY}.

    Since the construction of LEP as a $Z$ boson factory much progress has been
    made, particularly in the area of resonant states. In previous
    experiments resonances were measured with poor statistical precision
    and there were, in addition, some considerable systematic disagreements
    among experiments. The higher statistics obtainable at LEP are illustrated
    by Figure \ref{GLOB_XSEC}, which shows the much larger hadronic
    cross-section compared to the lower energy colliders: with a
    comparable luminosity, LEP has experienced much higher reaction rates   
    and since the startup of LEP in 1989 each of the four experiments,
    ALEPH, DELPHI, L3 and OPAL, has collected several million hadronic   
    $Z$ decays. 

%
\vspace{30mm}
\begin{figure}[htb]
\vspace{-15mm}
\begin{center}
\epsfig{file=figures/glob_xsec.eps,height=9cm}
\end{center}
\vspace{-1mm}
\caption[Total cross-section for $\ee \rightarrow \qq$.]
        {\label{GLOB_XSEC}
        {\it Total cross-section for $\ee$~annihilation
             into hadrons and muon pairs as function of the
             centre-of-mass energy.
             Also given is the two-photon cross-section.
             Experimental data are compared with predictions
             from the standard model.}}
\end{figure}
%


    More information can be gained by studying the production rates of
    resonances. Resonant states are particularly interesting because they
    are less likely than the lighter hadrons to be products of particle
    decays and therefore their dynamics are more closely related
    to those of the fragmenting partons. The light vector mesons are
    particularly well suited as they are copiously produced in hadronic
    events giving rise to a significant fraction of the observed stable
    particles. In addition, measurements of the vector mesons contribute
    to a more complete picture of particle production. Hence,
    the measurement of inclusive particle production cross sections
    of resonant states improve the description of the hadronisation
    process. The large sample of hadronic Z decays
    collected at LEP is ideal for this purpose.

    This study presents the ALEPH measurement \cite{ALEPH_RULE} of the rate 
    and differential cross section of the $\rho(770)^\pm$ meson produced in hadronic 
    Z decays.
    $\rho^\pm$ candidates are reconstructed from their daughter pions
    ($\rho^\pm \rightarrow \pi^0 \pi^\pm$, BR $\approx$ 100\%).
    The analysis described here is essentially similar to that of papers
    such as \cite{ALEPH_VMP} and \cite{OPAL_VMP}, and it is based on 
    about 3.2 million selected 
    hadronic events recorded by the ALEPH detector at centre-of-mass energies around 
    $\sqrt{s} = 91.2\unit{GeV}$ in the running period of LEP between 1991 and 1995.
    The results of the evaluated rates and cross sections are compared with
    Monte Carlo programs {\sc Jetset 7.4}, {\sc Pythia 6.4} and {\sc Herwig 6.5},  and 
    the OPAL measurement which is the only other experiment at LEP to 
    make this measurement. \\

    This thesis includes a short summary of the Standard Model,
    a theoretical description of the fragmentation models
    and a brief description of the experimental apparatus including the
    data acquisition system, event reconstruction, and detector simulation.
    The analysis is presented in Chapters 5 to 10, and the results and
    conclusions are given in Chapter 11.

%
% end chapter 1 : Introduction
%

